CRAFT: Customizing LLMs by Creating and Retrieving from Specialized Toolsets

Large language models (LLMs) are often augmented with tools to solve complex tasks. By generating code snippets and executing them through task-specific Application Programming Interfaces (APIs), they can offload certain functions to dedicated external modules, such as image encoding and performing calculations. However, most existing approaches to augment LLMs with tools are constrained by general-purpose APIs and lack the flexibility for tailoring them to specific tasks. In this work, we present CRAFT, a general tool creation and retrieval framework for LLMs. It creates toolsets specifically curated for the tasks and equips LLMs with a component that retrieves tools from these sets to enhance their capability to solve complex tasks. For each task, we collect specific code solutions by prompting GPT-4 to solve the training examples. Following a validation step ensuring the correctness, these solutions are abstracted into code snippets to enhance reusability, and deduplicated for higher quality. At inference time, the language model retrieves snippets from the toolsets and then executes them or generates the output conditioning on the retrieved snippets. Our method is designed to be flexible and offers a plug-and-play approach to adapt off-the-shelf LLMs to unseen domains and modalities, without any finetuning. Experiments on vision-language, tabular processing, and mathematical reasoning tasks show that our approach achieves substantial improvements compared to strong baselines. In addition, our in-depth analysis reveals that: (1) consistent performance improvement can be achieved by scaling up the number of tools and the capability of the backbone models; (2) each component of our approach contributes to the performance gains; (3) the created tools are well-structured and reliable with low complexity and atomicity. The code is available at https://github.com/lifan-yuan/CRAFT.

==> figs_latex/toolbase_construction.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figs/toolbase_construction.pdf}
    \caption{The construction pipeline of tool base. \lifan{draft} \xingyao{I feel it will be nice if you merge fig.1 and fig.2. Basically it will be a large figure with two boxes, one being tool construction, and another being tool retrieval. And you can connect these two big boxes using an arror to show that they are in a same pipeline. It will probably make better use of space.}}
    \label{fig:toolbase_construction}
\end{figure}

==> figs_latex/wordcloud.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figs/wordcloud.pdf}
    \caption{The word cloud of function names in the tool base. \hao{don't think this visual provides any insights. we should consider moving it to the appendix}}
    \label{fig:wordcloud}
\end{figure}

==> section/formulation.tex <==
\section{Task Formulation}

Each complex task $t_i$ can be considered as a function that $f: x \in \mathcal{X} \rightarrow y \in \mathcal{Y}$, which can be decomposed into sub-tasks (functions) in arbitrary ways where the output of some sub-tasks will be the input of others, creating a tree of function calls, for example, $y = f(x) = f_3(f_1(x), f_2(x), x)$ as shown in Fig. \ref{fig:task-decomposition}.

\paragraph{Multiple Input-Output Pairs Per Task}
Similar to software engineering setting, we can have multiple valid input-output pairs for each task $t_i$. $\mathcal{X}$ is the space of all possible inputs and $\mathcal{Y}$ is the space for outputs.

% \paragraph{Nature of Inputs and Outputs}

\paragraph{One-Step Tasks}

Given a sets of complex tasks $t_i \in \mathcal{T}_{\texttt{complex}}$, we sample all the intermediate steps $f_1, f_2, \dots \textasciitilde f$ into a set of simple tasks $\mathcal{T}_{\texttt{simple}}$.

\paragraph{Test Cases / Verifier}

We need to design test cases to validate all the intermediate results (e.g., $f_1(x)$) to measure the correctness of the sub-task, as well as the final output $f(x)$.

\paragraph{Sub-task Decomposition}

We always design a sub-goal decomposition for each complex task (e.g., ground truth) and sample simple tasks from these ground truths.

Additionally, we have another evaluation model where we ask the LM itself to decompose the task.

\paragraph{File Archive}
Archive the relevant files as a copy to keep a static web search engine.


\begin{figure}[h]
    \centering
    % \includegraphics{}
\begin{tikzpicture}[level distance=1.5cm,
level 1/.style={sibling distance=3cm},
level 2/.style={sibling distance=1.5cm}]
\node {f(x)}
child {node {$f_3(\cdot, \cdot, \cdot)$}
child {node {$f_1(x)$}
child {node {$x$}}}
child {node {$f_2(x)$}
child {node {$x$}}}
child {node {$x$}}};
\end{tikzpicture}
\caption{Decomposing complex tasks into subtasks}
\label{fig:task-decomposition}
\end{figure}


\section{What to measure?}


\subsection{Complex Task Success Rate}

\paragraph{When sub-goal decomposition is given}
\paragraph{When sub-goal decomposition is NOT given (LM decomposed)}

\subsection{Simpler Task Success Rate}

\paragraph{Just success Rate}

\subsection{Additional Metrics}

\paragraph{Safety} Number of un-related files modified


==> tabs/scaling_model.tex <==
\begin{table*}[]
\centering
\caption{Ablation Study and Comparison between ViperGPT and \framework with GPT-4 being the backbone.}
\setlength{\tabcolsep}{9pt} % Default value: 6pt
\begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \multirow{2}{*}{GPT-4} & \multicolumn{2}{c}{OK-VQA}    &  & \multicolumn{2}{c}{GQA}       &  & \multicolumn{2}{c}{A-OKVQA}   \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-9} 
%                        & Acc           & F1            &  & Acc           & F1            &  & Acc           & F1            \\ \midrule
% ViperGPT               & 36.7          & 47.2          &  & 51.4          & 53.7          &  & 32.8          & 42.4          \\
% \framework              & \textbf{39.0} & \textbf{49.1} &  & \textbf{55.6} & \textbf{58.8} &  & \textbf{35.3} & \textbf{44.8} \\ \bottomrule
% \end{tabular}
\begin{tabular}{@{}llcc m{0.01em}  cc m{0.01em}  cc m{0.015em} @{}}
\toprule
\multicolumn{2}{l}{\multirow{2}{*}{GPT-3.5-Turbo}} & \multicolumn{2}{c}{\bf OK-VQA}    && \multicolumn{2}{c}{\bf \phantom{00}GQA\phantom{00}}       && \multicolumn{2}{c}{\bf A-OKVQA}   \\ 

\cline{3-4}
\cline{6-7}
\cline{9-10}

\multicolumn{2}{l}{}                               & Acc           & F1            && Acc           & F1            && Acc           & F1            \\ 


\midrule
\multicolumn{2}{l}{ViperGPT}                       & 36.7          & 47.2          && 51.4          & 53.7          && 32.8          & 42.4          \\
\multicolumn{2}{l}{\framework}                      & \textbf{39.0} & \textbf{49.1} && \textbf{55.6} & \textbf{58.8} && \textbf{35.3} & \textbf{44.8} \\ \cmidrule(l){3-10} 
                 & w/o Abstraction                 & 31.0          & 41.4          && 37.1          & 39.7          && 28.0          & 39.3          \\
                 & w/o Query                       & 32.7          & 42.3          && 42.4          & 45.8          && 29.8          & 38.7          \\
                 & w/o Name                        & 26.8          & 35.7          && 36.4          & 38.3          && 21.7          & 30.6          \\
                 & w/o Docstring                   & 29.8          & 38.8          && 37.3          & 39.1          && 25.0          & 34.0          \\ \midrule
\multicolumn{2}{l}{\multirow{2}{*}{GPT-4}}         & \multicolumn{2}{c}{\bf OK-VQA}    && \multicolumn{2}{c}{\bf \phantom{00}GQA\phantom{00}}       && \multicolumn{2}{c}{\bf A-OKVQA}   \\ 

\cline{3-4}
\cline{6-7}
\cline{9-10}

\multicolumn{2}{l}{}                               & Acc           & F1            && Acc           & F1            && Acc           & F1            \\ 


\midrule
\multicolumn{2}{l}{ViperGPT}                       & 36.7          & 47.2          && 51.4          & 53.7          && 32.8          & 42.4          \\
\multicolumn{2}{l}{\framework}                      & \textbf{39.0} & \textbf{49.1} && \textbf{55.6} & \textbf{58.8} && \textbf{35.3} & \textbf{44.8} \\ \bottomrule
\end{tabular}
\end{adjustbox}

\label{tab:scaling_model}
\end{table*}

==> tabs/scaling_toolbase.tex <==
\begin{table}[]
\centering
\caption{Results of scaling tool base (will change to fig)}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Epoch} & \multicolumn{3}{c|}{OK-VQA}                  & \multicolumn{3}{c|}{GQA}                     & \multicolumn{3}{c}{AOK-VQA}                  \\ \cmidrule(l){2-10} 
                       & Acc            & F1             & TUR & Acc            & F1             & TUR & Acc            & F1             & TUR \\ \midrule
0                      & 15.43          & 24.71          & 0.00       & 35.00          & 36.90          & 0.00       & 15.63          & 23.04          & 0.00       \\
1                      & 30.90          & 40.50          & 25.90      & 40.70          & 43.17          & 17.10      & 25.07          & 36.39          & 31.20      \\
4                      & 32.07          & 41.86          & 26.50      & 42.00          & 44.89          & 14.60      & 26.13          & 37.44          & 32.30      \\
7                      & 28.70          & 38.89          & 25.00      & 40.60          & 42.81          & 14.40      & 28.37          & 38.83          & 36.00      \\
10                     & \textbf{29.77} & \textbf{40.17} & 26.70      & \textbf{42.30} & \textbf{45.20} & 12.90      & \textbf{28.13} & \textbf{38.48} & 31.70      \\
11                     & 33.43          & 43.03          & 24.50      & 45.40          & 48.75          & 12.30      & 30.80          & 40.63          & 33.20      \\ \bottomrule
\end{tabular}

}

\label{tab:my-table}
\end{table}
